A Stochastic Operator Approach to Model Inadequacy with Applications to Contaminant Transport

The mathematical models used to represent physical phenomena are generally known to be imperfect representations of reality. Model inadequacies arise for numerous reasons, such as incomplete knowledge of the phenomena or computational intractability of more accurate models. In such situations it is impractical or impossible to improve the model, but necessity requires its use to make predictions. With this in mind, it is important to represent the uncertainty that a model's inadequacy causes in its predictions, as neglecting to do so can cause overconfidence in its accuracy. A powerful approach to addressing model inadequacy leverages the composite nature of physical models by enriching a flawed embedded closure model with a stochastic error representation. This work outlines steps in the development of a stochastic operator as an inadequacy representation by establishing the framework for inferring an infinite-dimensional operator and by introducing a novel method for interrogating available high-fidelity models to learn about modeling error.

==> Makefile <==
#vectorsources := $(shell find rawfigs/ ../common/rawfigs/ -name '*.dia' -o -name '*.eps' -o -name '*.m' -o -name '*.pdf' -o -name '*.ps' -o -name '*.py' -o -name '*.svg' 2>/dev/null)
#rastersources := $(shell find rawfigs/ ../common/rawfigs/ -name '*.jpg' -o -name '*.gif' 2>/dev/null)
readysources := $(shell find rawfigs/ ../common/rawfigs/ -name '*.png' -o -name '*.pdf' -o -name '*mpg' -o -name '*.mpeg' 2>/dev/null)
#texsource := $(wildcard abstract.tex paper.tex poster.tex proposal.tex report.tex talk.tex)
texsource := $(wildcard paper.tex poster.tex proposal.tex report.tex talk.tex)

#vectorfigs := $(shell echo ' ' $(patsubst %_fm.eps,%.eps,$(vectorsources)) ' ' | sed -e 's> \(../common/\)*raw> >g' -e 's/\.[^. ]* /.pdf /g')
#rasterfigs := $(shell echo ' ' $(rastersources) ' ' | sed -e 's> \(../common/\)*raw> >g' -e 's/\.[^. ]* /.png /g')
readyfigs := $(shell echo ' ' $(readysources) ' ' | sed -e 's> \(../common/\)*raw> >g')
figsources := $(vectorsources) $(rastersources) $(readysources)
figures := $(vectorfigs) $(rasterfigs) $(readyfigs)
dirname  := $(shell basename $(shell pwd))
ifeq ($(words $(texsource)),'1')
    texfinal := $(dirname).pdf
    texroot   = $(patsubst %.pdf,%,$(1))
else
    texfinal := $(patsubst %.tex,$(dirname)-%.pdf,$(texsource))
    texroot   = $(patsubst $(dirname)-%,%,$(patsubst %.pdf,%,$(1)))
endif

bibfiles := $(wildcard *.bib)
styfiles := $(wildcard *.sty ../common/*.sty)
clsfiles := $(wildcard *.cls ../common/*.cls)

alldeps := *.tex $(bibfiles) $(figures) $(figsources) $(clsfiles) $(styfiles)

BIBTEX     ?= bibtex
PDFLATEX   ?= pdflatex
LATEX      ?= latex
PYTHON     ?= python
OCTAVE     ?= octave
INKSCAPE   ?= inkscape
FRAGMASTER ?= fragmaster

MYPDFLATEX   = TEXINPUTS=$(abspath ../common):$$TEXINPUTS $(PDFLATEX) -halt-on-error -interaction=nonstopmode
MYLATEX      = TEXINPUTS=$(abspath ../common):$$TEXINPUTS $(LATEX) -halt-on-error -interaction=nonstopmode
MYFRAGMASTER = TEXINPUTS=$(abspath ../common):$$TEXINPUTS $(FRAGMASTER)

.PHONY: all figures clean cleanlatex cleanfigs

all: $(texfinal)

figures: $(figures)

continuous: all
	while true; do \
	  inotifywait -e close_write -e delete_self -e move $(alldeps) || break; \
          $(MAKE) all; \
        done

$(texfinal): $(alldeps)
	if ls *.bib 2>&1; then $(MYPDFLATEX) -draftmode $(call texroot,$@); fi
	if (ls *.bib 2>&1 && ls $(call texroot,$@).aux 2>&1); then $(BIBTEX) $(call texroot,$@); fi
	$(MYPDFLATEX) -draftmode $(call texroot,$@) && $(MYPDFLATEX) -draftmode $(call texroot,$@) && $(MYPDFLATEX) $(call texroot,$@)
	if [ "$@" != "$(call texroot,$@).pdf" ]; then mv "$(call texroot,$@).pdf" "$@"; fi

clean: cleanlatex cleanfigs

cleanlatex:
	rm -f $(patsubst %.tex, %.aux, $(wildcard *.tex))
	#rm -f $(foreach ext,.bbl .blg .log .dvi .nav .nlo .out .pdf .snm .spl .toc .vrb Notes.bib,$(patsubst %.tex,%$(ext),$(texsource)))
	rm -f $(foreach ext, .blg .log .dvi .nav .nlo .out .pdf .snm .spl .toc .vrb Notes.bib,$(patsubst %.tex,%$(ext),$(texsource)))
	rm -f $(texfinal)

cleanfigs:
	rm -rf figs/

figs/%.pdf: rawfigs/%.dia
	@mkdir -p $(dir $@)
	dia -t eps-builtin -e $?_roytemp.eps $? && epstopdf $?_roytemp.eps -o=$@
	@rm -f $?_roytemp.eps

figs/%.pdf: rawfigs/%.eps
	@mkdir -p $(dir $@)
	epstopdf $? -o=$@ || (rm $@; exit 1)

figs/%.pdf: rawfigs/%_fm rawfigs/%_fm.eps  # fragmaster(1) with optional control file
	@mkdir -p $(dir $@)
	@(test -f rawfigs/fragmaster.dfm && (cd $(dir $@) && ln -sf -t . ../rawfigs/fragmaster.dfm) || true)
	@(cd $(dir $@) && ln -sf -t . $(addprefix ../,$+) && $(MYFRAGMASTER))

figs/%.pdf: rawfigs/%.m
	@mkdir -p $(dir $@)
	@cd $(dir $?) && $(OCTAVE) $(notdir $?)
	@(test -f $(dir $?)/$*.eps && (epstopdf $(dir $?)/$*.eps -o=$@; rm -f $(dir $?)/$*.eps) || true)
	@(test -f $(dir $?)/$*.pdf && mv $(dir $?)/$*.pdf $@ || true)

figs/%.pdf: rawfigs/%.py
	@mkdir -p $(dir $@)
	@cd $(dir $?) && $(PYTHON) $(notdir $?)
	@(test -f $(dir $?)/$*.eps && (epstopdf $(dir $?)/$*.eps -o=$@; rm -f $(dir $?)/$*.eps) || true)
	@(test -f $(dir $?)/$*.pdf && mv $(dir $?)/$*.pdf $@ || true)

figs/%.pdf: rawfigs/%.ps
	@mkdir -p $(dir $@)
	ps2pdf $? $@

#figs/%.pdf: rawfigs/%.png
#       convert $? $@

figs/%.pdf: rawfigs/%.svg
	@mkdir -p $(dir $@)
	$(INKSCAPE) $? -z --export-pdf=$@

figs/%.png: rawfigs/%.jpg
	@mkdir -p $(dir $@)
	convert $? $@

figs/%.png: ../common/rawfigs/%.jpg
	@mkdir -p $(dir $@)
	convert $? $@

figs/%.png: rawfigs/%.gif
	@mkdir -p $(dir $@)
	convert $? $@

figs/%.png: ../common/rawfigs/%.gif
	@mkdir -p $(dir $@)
	convert $? $@

figs/%.mpeg: rawfigs/%.mpeg
	@mkdir -p $(dir $@)
	@reldir=`echo $(dir $@) | sed -e 's>[^/]*/*>../>g'`; ln -sf $${reldir}$? $@

figs/%.mpg: rawfigs/%.mpg
	@mkdir -p $(dir $@)
	@reldir=`echo $(dir $@) | sed -e 's>[^/]*/*>../>g'`; ln -sf $${reldir}$? $@

figs/%.pdf: rawfigs/%.pdf
	@mkdir -p $(dir $@)
	@reldir=`echo $(dir $@) | sed -e 's>[^/]*/*>../>g'`; ln -sf $${reldir}$? $@

figs/%.png: rawfigs/%.png
	@mkdir -p $(dir $@)
	@reldir=`echo $(dir $@) | sed -e 's>[^/]*/*>../>g'`; ln -sf $${reldir}$? $@

figs/%.pdf: ../common/rawfigs/%.pdf
	@mkdir -p $(dir $@)
	@reldir=`echo $(dir $@) | sed -e 's>[^/]*/*>../>g'`; ln -sf $${reldir}$? $@

figs/%.png: ../common/rawfigs/%.png
	@mkdir -p $(dir $@)
	@reldir=`echo $(dir $@) | sed -e 's>[^/]*/*>../>g'`; ln -sf $${reldir}$? $@

figs/%.pdf: ../common/rawfigs/%.eps
	@mkdir -p $(dir $@)
	epstopdf $? -o=$@

figs/%.pdf: ../common/rawfigs/%.ps
	@mkdir -p $(dir $@)
	ps2pdf $? $@

figs/%.pdf: ../common/rawfigs/%.svg
	@mkdir -p $(dir $@)
	$(INKSCAPE) $? -z --export-pdf=$@

